Team Formation amidst Conflicts

In this work, we formulate the problem of team formation amidst conflicts. The goal is to assign individuals to tasks, with given capacities, taking into account individuals' task preferences and the conflicts between them. Using dependent rounding schemes as our main toolbox, we provide efficient approximation algorithms. Our framework is extremely versatile and can model many different real-world scenarios as they arise in educational settings and human-resource management. We test and deploy our algorithms on real-world datasets and we show that our algorithms find assignments that are better than those found by natural baselines. In the educational setting we also show how our assignments are far better than those done manually by human experts. In the human resource management application we show how our assignments increase the diversity of teams. Finally, using a synthetic dataset we demonstrate that our algorithms scale very well in practice.

==> images/macros.tex <==
% !TEX root = neurips_2020.tex

%proposal
\newcommand{\thresholdgreedy}{\texttt{Threshold}}
\newcommand{\greedy}{\texttt{Greedy}}
\newcommand{\continuous}{\texttt{Continuous}}
\newcommand{\reward}{\ensuremath{r}}
\newcommand{\vb}{\ensuremath{\vec{\beta}}}
\newcommand{\bx}{\ensuremath{\mathbf{x}}}
\newcommand{\be}{\ensuremath{\mathbf{e}}}
\newcommand{\ba}{\ensuremath{\mathbf{a}}}
\newcommand{\bw}{\ensuremath{\mathbf{w}}}
\newcommand{\tr}{\ensuremath{\text{tr}}}
\newcommand{\vc}{\ensuremath{\text{vec}}}
\newcommand{\evec}{\ensuremath{\mathbf{e}}}
\newcommand{\zerovec}{\ensuremath{\mathbf{0}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\bb}{\ensuremath{\mathbf{b}}}
\newcommand{\bo}{\ensuremath{\mathbf{o}}}
\newcommand{\bbeta}{\ensuremath{\boldsymbol{\beta}}}
\newcommand{\numexperts}{\ensuremath{n}}
\newcommand{\numtransformation}{\ensuremath{k}}
\newcommand{\experts}{\ensuremath{\Omega}}
\newcommand{\dataset}{\ensuremath{D}}
\newcommand{\constraints}{\calC}
\newcommand{\betconstr}{\calB}
\newcommand{\argmin}{\ensuremath{\mathop{\arg\min}}}
\newcommand{\argmax}{\ensuremath{\mathop{\arg\max}}}
\newcommand{\iloss}{\ell}
\newcommand{\etal}{\textit{et al.}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\naturals}{\ensuremath{\mathbb{N}}}
\newcommand{\diag}{\ensuremath{\mathop{\mathrm{diag}}}}
\newcommand{\alternative}{\texttt{Alternative 1}}
\newcommand{\newalt}{\texttt{Alternative 2}}
\newcommand{\bibsonomy}{\textit{Bibsonomy}}
\newcommand{\imdb}{\textit{IMDB}}
\newcommand{\nba}{\textit{NBA}}
\newcommand{\googlescholar}{\textit{GoogleScholar}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
% Problems
\newcommand{\setcover}{{\sc SetCover}}

% Algorithms

\newcommand{\MFW}{{\texttt{Mono-FW}}}
\newcommand{\BFW}{{\texttt{Bandit-FW}}}
\newcommand{\RFW}{{\texttt{Responsive-FW}}}
\newcommand{\OurAlgo}{{\texttt{General-Algorithm}}}
\newcommand{\MaxAlgo}{{\texttt{A}}}
\newcommand{\VE}{{\texttt{VE}}}
\newcommand{\Ex}{{\texttt{E}}}
\newcommand{\FindCuts}{{\texttt{ComputeCuts}}}
\newcommand{\FindEdges}{{\texttt{ComputeEdges}}}
\newcommand{\BallOne}{{\texttt{ConfidenceBall$_1$}}}

% Problem settings 
\newcommand{\DSMB}{{\texttt{DSMB}}}
\newcommand{\SSMF}{{\texttt{SSMF}}}
\newcommand{\SLOB}{{\texttt{SLOB}}}
\newcommand{\SSMB}{{\texttt{SSMB}}}

% Function
\newcommand{\dist}{\ensuremath{d}}
\newcommand{\zfunc}{\ensuremath{\mathbf{z}}}
\newcommand{\zfuncx}{\ensuremath{\zfunc(\xvec)}}
\newcommand{\zfuncz}{\ensuremath{\zfunc(\zvec)}}
\newcommand{\zfunce}{\ensuremath{\zfunc(\evec)}}
\newcommand{\zfunct}{\ensuremath{\zfunc(\xvec_t)}}
\newcommand{\zfunctau}{\ensuremath{\zfunc(\xvec_{\tau})}}
\newcommand{\zfuncapprox}{\ensuremath{\zfunc\left(\MaxAlgo\left( \wvec \right)\right)}}
\newcommand{\zfuncapproxm}{\ensuremath{\zfunc\left(\MaxAlgo\left( \muvec \right)\right)}}
\newcommand{\zfuncapproxe}{\ensuremath{\zfunc\left(\MaxAlgo\left( \evec \right)\right)}}
\newcommand{\zfuncopt}{\ensuremath{\zfunc(\xvec^{*})}}
\newcommand{\gfuncx}{\ensuremath{g(\xvec)}}
\newcommand{\gfunc}{\ensuremath{g}}
\newcommand{\gfuncs}{\ensuremath{g}}
\newcommand{\rfuncx}{\ensuremath{W(\xvec)}}
\newcommand{\rfuncn}{\ensuremath{W(\mathcal{N})}}
\newcommand{\rfunc}{\ensuremath{W}}
\newcommand{\rfuncs}{\ensuremath{W}}
\newcommand{\ffunc}{\ensuremath{f}}
\newcommand{\ffuncx}{\ensuremath{f(\xvec)}}
\newcommand{\ffunce}{\ensuremath{f(\evec)}}
\newcommand{\ffuncxopt}{\ensuremath{f(\xvec^{*})}}
\newcommand{\ffuncxg}{\ensuremath{f_G(\xvec)}}
\newcommand{\ffuncxy}{\ensuremath{f(\xvec,\yvec)}}
\newcommand{\ffunct}{\ensuremath{f(\xvec_t)}}
\newcommand{\xopt}{\ensuremath{\xvec^{*}}}
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\matroid}{\ensuremath{\mathcal{M}}}
\newcommand{\bone}{\ensuremath{\boldsymbol{1}}}

% Paragraphs
\newcommand{\spara}[1]{\smallbreak\noindent{\bf{#1}}}
\newcommand{\mpara}[1]{\medskip\noindent{\bf{#1}}}
\newcommand{\bpara}[1]{\bigskip\noindent{\bf{#1}}}
\newcommand{\para}{\smallbreak\noindent}
% \newcommand{\etal}{{et al.}}

% Operators + Latex related
 \newtheorem{assumption}{Assumption}
\newtheorem{observation}{Observation}

\newcommand*{\belowrulesepcolor}[1]{%
	\noalign{%
		\kern-\belowrulesep
		\begingroup
		\color{#1}%
		\hrule height\belowrulesep
		\endgroup
	}%
}
\newcommand*{\aboverulesepcolor}[1]{%
	\noalign{%
		\begingroup
		\color{#1}%
		\hrule height\aboverulesep
		\endgroup
		\kern-\aboverulesep
	}%
}


%% squishlist                                                                                                                    \                                                   

\newcommand{\squishlist}{\begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }
\newcommand{\squishend}{
  \end{list}  }

\newcommand{\regret}{\ensuremath{\mathcal{R}}}



==> sections/experiments_lab_times.tex <==
\note[ET]{Merge this with whatever you had above}
\subsection{Project preferences and time conflicts}

% In this scenario each student gives project preferences and declares available time slots chosen from a fixed list of time slots.
% The goal is to form teams so that students assigned to the same project have overlap in available time slots. In this way they can collaborate more efficiently.

% Setting the project preferences is the same as in the previous application.
% We add a conflict edge between two students $u$ and $v$ if they don't have a common time slot and set $w_{uv} = 1$.

